Spatial coupling of an explicit temporal adaptive integration scheme with an implicit time integration scheme

The Reynolds-Averaged Navier-Stokes equations and the Large-Eddy Simulation equations can be coupled using a transition function to switch from a set of equations applied in some areas of a domain to the other set in the other part of the domain. Following this idea, different time integration schemes can be coupled. In this context, we developed a hybrid time integration scheme that spatially couples the explicit scheme of Heun and the implicit scheme of Crank and Nicolson using a dedicated transition function. This scheme is linearly stable and second-order accurate. In this paper, an extension of this hybrid scheme is introduced to deal with a temporal adaptive procedure. The idea is to treat the time integration procedure with unstructured grids as it is performed with Cartesian grids with local mesh refinement. Depending on its characteristic size, each mesh cell is assigned a rank. And for two cells from two consecutive ranks, the ratio of the associated time steps for time marching the solutions is $2$. As a consequence, the cells with the lowest rank iterate more than the other ones to reach the same physical time. In a finite-volume context, a key ingredient is to keep the conservation property for the interfaces that separate two cells of different ranks. After introducing the different schemes, the paper recalls briefly the coupling procedure, and details the extension to the temporal adaptive procedure. The new time integration scheme is validated with the propagation of 1D wave packet, the Sod's tube, and the transport of a bi-dimensional vortex in an uniform flow.

==> 6_section.tex <==
% !TEX root = TI.tex
\section{Results for 2D/3D test cases}

==> 8_TVD_AION.tex <==
% !TEX root = TA.tex
\section{TVD property of hybrid part of AION scheme \label{sec:TVD_AION}}
In the following, conditions for TVD property are proved to be equivalent for TN scheme and the hybrid part of the AION scheme.
For the linear one-dimensional advection equation (see Eq.~\eqref{conv}) time integrated by hybrid part of AION scheme
(see Eq.\eqref{eq:AION_NHRM}
) such as:
\begin{equation}
\begin{aligned}
y^{n+1}=y^n-\nu_j(y_{j+1/2}-y_{j-1/2})
\end{aligned}
\label{eq:hybrid_1D_TVD_1}
\end{equation}
with $\nu_j=\frac{c\Delta t}{\Delta x_j}$. The face values can be written as
\begin{equation}
\begin{aligned}
y_{j+1/2}=&\omega_i y_j +\frac{1-\omega_j\nu_j}{2} \phi_j (\nabla_x)^n_{j+1/2} + \bigg(\omega_j-\frac{1}{2}\bigg)\phi_j(\widehat{\nabla}_x)_{j+1/2} \\
&(1-\omega_j)\bigg[ y^{n+1}_j+\frac{1}{2}\phi_j(\nabla_x)^{n+1}_{j+1/2}-\frac{1-\omega_j}{2}\psi_j(\Delta_t)^{n+1}_j\bigg]
\end{aligned}
\label{eq:hybrid_1D_TVD_2}
\end{equation}
with
\begin{equation}
\begin{aligned}
(\nabla_x)^n_{j+1/2}&=y^{n}_{j+1}-y^{n}_{j}\\
(\nabla_x)^{n+1}_{j+1/2}&=y^{n+1}_{j+1}-y^{n+1}_{j}\\
(\widehat{\nabla}_x)_{j+1/2}&=\widehat{y}_{j+1}-\widehat{y}_{j} \\
(\Delta_t)^{n+1}_j&=y^{n+1}_j-y^{n}_j,
\end{aligned}
\end{equation}
The functions $\phi_j$ and $\psi_j$ are respectively the spatial and temporal limiter
functions of $q_j=\frac{(\nabla_x)_{j-1/2}}{(\nabla_x)_{j+1/2}}$ and $s_j=\frac{(\Delta_t)_{j+1}}{(\nabla_x)_{j}}$.
By substitution of the above Eq.~\eqref{eq:hybrid_1D_TVD_2} into Eq.~\eqref{eq:hybrid_1D_TVD_1},
the following formulation of the hybrid time integration is obtained:
\begin{equation}
\begin{aligned}
y^{n+1}_{j}=&y^{n}_j-\nu_j\bigg[ \omega_j (\nabla_x)^n_{j-1/2} +(1-\omega_j)(\nabla_x)^{n+1}_{j-1/2}-\frac{(1-\omega_j)^2}{2}\big[ \psi_{j}-\frac{\psi_{j-1}}{s_{j-1}} \big] (\Delta_t)^{n+1}_j \\
& +\frac{1-\omega_j^2\nu_j}{2}\big[ \frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^n(\nabla_x)^{n}_{j-1/2} +(\omega_j-\frac{1}{2})\big[ \frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^{\widehat{}}  (\widehat{\nabla}_x)_{j-1/2}\\
&+\frac{1-\omega_j}{2}\big[ \frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^{n+1}(\nabla_x)^{n+1}_{j-1/2}
\bigg]
\end{aligned}
\label{eq:hybrid_1D_TVD_3}
\end{equation}
Then with some rearrangement that leads to:
\begin{equation}
\begin{aligned}
\big(y^{n+1}_{j}-y^{n}_j\big)\bigg[ 1+\frac{\nu_j(1-\omega_j)^2}{2}\big[ \frac{\psi_{j-1}}{s_{j-1}}-\psi_{j} \big] \bigg]=&-\nu_j\bigg[ \omega_j+\frac{1-\omega_j^2\nu_j}{2}\big[ \frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^n\bigg](\nabla_x)^n_{j-1/2}\\
&-\nu_j\bigg[ (\omega_j-\frac{1}{2})\big[ \frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^{\widehat{}}\bigg]  (\widehat{\nabla}_x)_{j-1/2}\\
&-\nu_j(1-\omega_j)\bigg[1+\frac{1}{2}\big[ \frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^{n+1}\bigg](\nabla_x)^{n+1}_{j-1/2}
\end{aligned}
\label{eq:hybrid_1D_TVD_4}
\end{equation}
Defining the parameter $\beta$ as
\begin{equation}
\begin{aligned}
\beta=1+\frac{\nu_j(1-\omega_j)^2}{2}\big[\frac{\psi_{j-1}}{s_{j-1}}-\psi_{j}\big],
\end{aligned}
\label{eq:beta}
\end{equation}
and substituting Eq.~\eqref{eq:beta} in Eq.~\eqref{eq:hybrid_1D_TVD_4}:
\begin{equation}
\begin{aligned}
y^{n+1}_{j}+\frac{\nu_j(1-\omega_j)}{\beta}\bigg[1+\frac{1}{2}\big[ \frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^{n+1}\bigg](\nabla_x)^{n+1}_{j-1/2} =&y^{n}_j-\frac{\nu_j}{\beta}\bigg[ (\omega_j-\frac{1}{2})\big[ \frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^{\widehat{}}\bigg]  (\widehat{\nabla}_x)_{j-1/2}\\
&-\frac{\nu_j}{\beta}\bigg[ \omega_j+\frac{1-\omega_j^2\nu_j}{2}\big[ \frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^n\bigg](\nabla_x)^n_{j-1/2}\\
\end{aligned}
\label{eq:hybrid_1D_TVD_5}
\end{equation}
Equation~\eqref{eq:hybrid_1D_TVD_5} may be reformulated as:
\begin{equation}
\begin{aligned}
y^{n+1}_{j}-A(\nabla_x)^{n+1}_{j-1/2} =&y^{n}_j-B(\nabla_x)^n_{j-1/2}-C(\widehat{\nabla}_x)_{j-1/2}\\
\end{aligned}
\label{eq:hybrid_1D_TVD_6}
\end{equation}
According to Harten's theorem, the sufficient conditions for Eq.~\eqref{eq:hybrid_1D_TVD_6} are:
\begin{equation}
\left\{
\begin{array}{ll}
A \leq 0 \\
0\leq B+C \leq 1\\
\end{array}
\right.
\label{eq:Harten_condition}
\end{equation}
with:
\begin{equation}
\begin{aligned}
A&=-\frac{\nu_j(1-\omega_j)}{\beta}\bigg[1+\frac{1}{2}\big[ \frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^{n+1}\bigg]\\
B&= \frac{\nu_j}{\beta}\bigg[ \omega_j+\frac{1-\omega_j^2\nu_j}{2}\big[ \frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^n\bigg]\\
C&=\frac{\nu_j}{\beta}\bigg[ (\omega_j-\frac{1}{2})\big[ \frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^{\widehat{}}\bigg]
\end{aligned}
\label{eq:ABC}
\end{equation}
Applying the condition \eqref{eq:Harten_condition} and considering $A\leq0$ then
\begin{equation}
A\leq0 \Rightarrow
\left\{
\begin{array}{ll}
1+\frac{1}{2}\big[ \frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^{n+1} \geq 0 \\
\frac{(1-\omega_j)\nu_j}{\beta} \geq 0\\
\end{array}
\right.\label{eq:inegality_1}
\end{equation}
The first inequality in Eq.~\eqref{eq:inegality_1} is satisfied by the space limiter such as minmod~\cite{Roe_1986_ARFM}.
Then according to the second inequality in Eq.~\eqref{eq:inegality_1}, the first condition on time limiter to be TVD is
\begin{equation}
\begin{aligned}
\frac{\psi_{j-1}}{s_{j-1}}-\psi_{j}\geq - \frac{2}{\nu_j(1-\omega_j)^2}
\end{aligned}
\label{eq:N1}
\end{equation}
The other condition to be TVD according to Eq.~\eqref{eq:Harten_condition} leads to:
\begin{equation}
B+C\geq0 \Rightarrow
\left\{
\begin{array}{ll}
\nu_j\bigg(\omega_j+\frac{1-\omega_j^2\nu_j}{2}\big[ \frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^{n}+(\omega_j-\frac{1}{2})\big[ \frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^{\widehat{}}\bigg) \geq 0 \\
1+\frac{(1-\omega_j)^2\nu_j}{2}\big[ \frac{\psi_{j-1}}{s_{j-1}}-\psi_{j} \big] \geq 0\\
\end{array}
\right.\label{eq:inegality_2}
\end{equation}
The first inequality in Eq.~\eqref{eq:inegality_2} is satisfy for any space limiter
(e.g. minmod limiter) as long as $\nu_j\omega_j\leq 1$ and $0.6<\omega_j<1$.
The second inequality results in the same condition on time limiter (see Eq.~\eqref{eq:N1}).
The last condition for TVD leads to:
\begin{equation}
B+C\leq1 \Rightarrow
\begin{array}{ll}
 \frac{\nu_j\bigg(\omega_j+\frac{1-\omega_j^2\nu_j}{2}\big[ \frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^{n}+(\omega_j-\frac{1}{2})\big[ \frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^{\widehat{}}\bigg)}{1+\frac{(1-\omega_j)^2\nu_j}{2}\big[ \frac{\psi_{j-1}}{s_{j-1}}-\psi_{j} \big]} \leq 1 \\
\end{array}
\label{eq:inegality_3}
\end{equation}
According to the fact that maximum value for $\big[ \frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^{n}$ and $\big[\frac{\phi_{j}}{q_{j}}-\phi_{j-1} \big]^{\widehat{}}$ for space limiter is $2$ leads to same condition for time limiter than TN scheme for TVD property:
\begin{equation}
\begin{aligned}
\frac{\psi_{j-1}}{s_{j-1}}-\psi_{j}\geq - \frac{2}{\nu_j} \frac{1-\omega_j\nu_j(2-\omega_j\nu_j)}{(1-\omega_j)^2}
\end{aligned}
\label{eq:N2}
\end{equation}
This condition resulting from Eq.~\eqref{eq:N2} is more restrictive than condition from Eq.~\eqref{eq:N1},
and that is the only condition to satisfy to allow TVD property for the hybrid part of the AION scheme.















==> 9_demo_AION_accuracy.tex <==
\section{Time Accuracy with AION scheme\label{AION+TA_accuracy}}
Current section deals with the local analysis of time accuracy for the temporal adaptive method coupled with AION scheme near a interface concerned by time synchronisation thanks to hybrid part of the AION scheme.
For this, the finite-volume formulation of an one-dimensional ODE (see Eq.~\eqref{eq:EDP_order}) is considered.
Considering a $p^{\mbox{\scriptsize th}}$-order accurate spatial numerical scheme and
the predictor step of the hybrid part of AION time integrator that is first-order time accurate (see Eq.~\eqref{eq:HCS2}),
Eq.~\eqref{eq:EDP_order} may be written as (omitting subscript $j$)
\begin{equation}
\widehat{W}^{\omega \Delta t} = {W}^{0} + \omega\Delta t \big( \mathcal{R} + \mathcal{O}(\Delta x^{p-1}) \big) + \mathcal{O}(\Delta t^{2})
= {W}^{0} + \omega \Delta t \mathcal{R} + \mathcal{O}(\Delta t \Delta x^{p-1}, \Delta t^{2}).
\label{eq:predictor_AION}
\end{equation}

Firstly the local error performed at cells of class rank $1$ will be study.
\subsubsection{Local numerical error of cells of class rank $1$}
Thanks to the numerical error performed at predictor state (see Eq.~\eqref{eq:predictor_AION}) and expansion of reconstruction in hybrid part of AION scheme (see eq.\ref{eq:AION_NHRM}), it is possible to rewrite the expression of hybrid flux (omitting subscript of interface index) such as:
\begin{equation}
\begin{aligned}
F^{Hybrid}(\widehat{W}^{2\omega\Delta t})&=F\bigg(\omega \bigg\{\frac{W^0+\widehat{W}^{2\omega\Delta t}}{2}\bigg\}+\mathcal{O}(\Delta x^{p}) \\
&\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }+(1-\omega)\bigg\{W^0+2\Delta t\frac{\partial \mathcal{W}}{\partial t}-\frac{1-\omega}{2}2\Delta t\frac{\partial \mathcal{W}}{\partial t}+\mathcal{O}(\Delta t^{2},\Delta x^p)\bigg\} \bigg) \\
&=F\bigg(W^0+\Delta t\frac{\partial \mathcal{W}}{\partial t}+\mathcal{O}(\Delta t^2,\Delta x^{p}) +\frac{\omega}{2}\bigg\{\mathcal{O}(\Delta t^2,\Delta t\Delta x^{p-1})\bigg\} \bigg) \\
&=\mathcal{F}\bigg(W^0+\Delta t\frac{\partial \mathcal{W}}{\partial t}+\mathcal{O}(\Delta t^2,\Delta x^{p}) +\frac{\omega}{2}\bigg\{\mathcal{O}(\Delta t^2,\Delta t\Delta x^{p-1})\bigg\} \bigg)+\mathcal{O}(\Delta x^{p}).
\end{aligned}
\label{eq:flux_exp_AION}
\end{equation}
Thus the hybrid residual may be reformulate thanks to Eqs.~\eqref{eq:flux_exp_AION} and~\eqref{eq:EDP_order}:
%Then according to Eqs.~\eqref{eq:flux_exp_AION} and~\eqref{eq:EDP_order}, it is possible to formulate the residual as
\begin{equation}
\begin{aligned}
R^{Hybrid}(\widehat{W}^{2\omega\Delta t})&=\mathcal{R}\bigg(W^0+\Delta t\frac{\partial \mathcal{W}}{\partial t}+\mathcal{O}(\Delta t^2,\Delta x^{p}) +\frac{\omega}{2}\bigg\{\mathcal{O}(\Delta t^2,\Delta t\Delta x^{p-1})\bigg\} \bigg)+\mathcal{O}(\Delta x^{p-1}).
\end{aligned}
\end{equation}
Assumming that there are no numerical error at instant $t=0$ (i.e. $W^0=\mathcal{W}^0$ and also $\mathcal{R}=\mathcal{R}(W^0)$ in the following),
the Taylor expansion of hybrid flux (omitting subscript of interface index) around $W^0$ leads to
\begin{equation}
\begin{aligned}
F^{Hybrid}(\widehat{W}^{2\omega\Delta t})=\mathcal{F}+\Delta t \mathcal{R} \frac{\partial \mathcal{F}}{\partial \mathcal{W}}+\mathcal{O}({\Delta t^2},\Delta t\Delta x^{p-1},\Delta x^{p}).
\end{aligned}
\label{eq:error_flux_2dt_AION}
\end{equation}
Thanks to Eqs.~\eqref{eq:error_flux_2dt_AION} and~\eqref{eq:EDP_order}, the hybrid residual is reformulated as
\begin{equation}
\begin{aligned}
R^{Hybrid}(\widehat{W}^{2\omega\Delta t})=\mathcal{R}+\Delta t \mathcal{R} \frac{\partial \mathcal{R}}{\partial \mathcal{W}}+\mathcal{O}(\frac{\Delta t^2}{\Delta x},\Delta t\Delta x^{p-2},\Delta x^{p-1}).
\end{aligned}
\label{eq:error_residual_2dt_AION}
\end{equation}
Then state $W$ at cells of class rank $1$ may be formulated such as
\begin{equation}
\begin{aligned}
W^{2\Delta t}&={W}^{0}+{2\Delta t} \big( R^{Hybrid}(\widehat{W}^{2\omega\Delta t})\big). \\
&={W}^{0}+{2\Delta t} \bigg(  \mathcal{R}+\Delta t \mathcal{R} \frac{\partial \mathcal R}{\partial \mathcal{W}}+\mathcal{O}(\frac{\Delta t^2}{\Delta x},\Delta t\Delta x^{p-2},\Delta x^{p-1}) \bigg). \\
\end{aligned}
\end{equation}
Thus the numerical error of $W^{2\Delta t}$ at cells of class rank $1$ may be formulate such as
%Hence it is possible to formulate the numerical error of $W^{2\Delta t}$ at cells of class rank $1$,
\begin{equation}
\begin{aligned}
    e(W^{2\Delta t})&=\mathcal{W}^{0}+2\Delta t\frac{\partial \mathcal{W}}{\partial t}+2{\Delta t^2}\frac{\partial^2 \mathcal{W}}{\partial t^2}+\mathcal{O}(\Delta t^3)-W^{2\Delta t} =\mathcal{O}(\Delta t^3,\frac{\Delta t^3}{\Delta x},\Delta t^2\Delta x^{p-2},\Delta t\Delta x^{p-1}).
\end{aligned}
\label{eq:error_classes_3_AION}
\end{equation}

As presented in the previous methodology of adaptive time integration (see sec.\ref{sec:TA_method_AION}),
the flux at interface $\beta-\frac{1}{2}$ has a special treatment.
The MUSCL reconstruction deals with a special treatment of cells of class rank $1$ depending on the stencil (see Step 4).
Here only cells $\beta+1$ of class rank $1$ are considered, so it is important to evaluate the impact of the parabolic interpolation on local numerical error.
The state $\widehat{W}^{\omega\Delta t}_{\beta+1}$ may be formulated thanks to Eq.~\eqref{eq:error_residual_2dt_AION}, such as: 

\begin{equation}
\begin{aligned}
\widehat{W}^{\omega\Delta t}_{\beta+1}&={W}^{0}_{\beta+1}+{\omega\Delta t} \bigg( \frac{3}{4}R(W^0)+\frac{1}{4}R^{Hybrid}(\widehat{W}^{2\omega\Delta t})\bigg). \\
&={W}^{0}_{\beta+1}+{\omega\Delta t}\bigg( \frac{3}{4}(\mathcal{R}+\mathcal{O}(\Delta x^{p-1})) +\frac{1}{4}(\mathcal{R}+\Delta t \mathcal{R} \frac{\partial \mathcal R}{\partial \mathcal{W}}+\mathcal{O}(\frac{\Delta t^2}{\Delta x},\Delta t\Delta x^{p-2},\Delta x^{p-1})\big) \bigg). \\
\end{aligned}
\label{eq:state_parabolic_AION}
\end{equation}
According to eq.\ref{eq:state_parabolic_AION} the error $e(\widehat{W}^{\omega\Delta t}_{\beta+1})$ may be formulated such as,
\begin{equation}
\begin{aligned}
    e(\widehat{W}^{\omega\Delta t}_{\beta+1})&=\mathcal{W}^{0}_{\beta+1}+\omega\Delta t\frac{\partial \mathcal{W}}{\partial t}+\frac{\omega^2\Delta t^2}{2}\frac{\partial^2 \mathcal{W}}{\partial t^2}+\mathcal{O}(\Delta t^{3})-\widehat{W}^{\omega\Delta t}_{\beta+1} \\
    &=\frac{\omega^2\Delta t^2}{2}\frac{\partial^2 \mathcal{W}}{\partial t^2}-\frac{\Delta t^2}{4}\mathcal{R} \frac{\partial \mathcal R}{\partial \mathcal{W}}+\mathcal{O}(\Delta t^3,\frac{\Delta t^3}{\Delta x},\Delta t^2\Delta x^{p-2},\Delta t\Delta x^{p-1}) \\
    &=\mathcal{O}(\Delta t^2,\frac{\Delta t^3}{\Delta x},\Delta t^2\Delta x^{p-2},\Delta t\Delta x^{p-1}).
\end{aligned}
\label{eq:error_parabolic_AION}
\end{equation}
This formulation of the error (Eq.~\eqref{eq:error_parabolic_AION}), lead to reformulate the numerical flux at interface $\beta-\frac{1}{2}$ such as:
\begin{equation}
\begin{aligned}
    F^{Hybrid}_{\beta-\frac{1}{2}}(\widehat{W}^{\Delta t})&=\mathcal{F}_{\beta-\frac{1}{2}}+\frac{\Delta t}{2} \mathcal{R} \frac{\partial \mathcal{F}_{\beta-\frac{1}{2}}}{\partial \mathcal{W}}+ \mathcal{O}(\Delta t^2,\frac{\Delta t^3}{\Delta x},\Delta t\Delta x^{p-2},\Delta x^{p-1}). \\
    F_{\beta-\frac{1}{2}}({W}^{0})&= \mathcal{F}_{\beta-\frac{1}{2}}+ \mathcal{O}(\Delta x^p).
\end{aligned}
\label{eq:error_flux_beta-1/2_AION}
\end{equation}

Now let us study the local numerical error of cell $\beta$ of class rank $0$.
\subsubsection{Local numerical error of cells $\beta$ of class rank $0$}
It is possible to rewrite the expression of hybrid flux (omitting subscript of interface index), according the numerical error performed at predictor state (see Eq.~\eqref{eq:predictor_AION}), such as:
\begin{equation}
\begin{aligned}
    F^{Hybrid}_{\beta+\frac{1}{2}}(\widehat{W}^{2\omega\Delta t})&=\mathcal{F}_{\beta+\frac{1}{2}}+\Delta t \mathcal{R} \frac{\partial \mathcal{F}_{\beta+\frac{1}{2}}}{\partial \mathcal{W}}+\mathcal{O}(\Delta t^2,\Delta t\Delta x^{p-1},\Delta x^{p}) .\\
    F_{\beta+\frac{1}{2}}({W}^{0})&= \mathcal{F}_{\beta+\frac{1}{2}}+ \mathcal{O}(\Delta x^p).
\end{aligned}
\label{eq:error_flux_beta_AION}
\end{equation}
Then the flux $F^{Hybrid}_{\beta+\frac{1}{2}}(\widehat{W}^{\omega\Delta t})$ may be formulated such as

\begin{equation}
\begin{aligned}
    F^{Hybrid}_{\beta+\frac{1}{2}}(\widehat{W}^{\omega\Delta t})&=\frac{1}{2} \bigg( F_{\beta+\frac{1}{2}}({W}^{0})+F^{Hybrid}_{\beta+\frac{1}{2}}(\widehat{W}^{2\omega\Delta t})\bigg)\\
    &=\mathcal{F}_{\beta+\frac{1}{2}}+ \frac{\Delta t}{2} \mathcal{R} \frac{\partial \mathcal{F}_{\beta+\frac{1}{2}}}{\partial \mathcal{W}}+\mathcal{O}(\Delta t^2,\Delta t\Delta x^{p-1},\Delta x^{p}) \\
\end{aligned}
\label{eq:error_flux_beta_2_AION}
\end{equation}

Thanks to Eqs.~\eqref{eq:error_flux_beta-1/2_AION}, \eqref{eq:error_flux_beta_2_AION}, and~\eqref{eq:error_flux_beta_AION},
the state $W^{\Delta t}_{\beta}$ may be formulated such as
\begin{equation}
\begin{aligned}
{W}^{\Delta t}_{\beta}&={W}^{0}_{\beta}+\frac{\Delta t}{\Delta x} \bigg( F^{Hybrid}_{\beta+\frac{1}{2}}(\widehat{W}^{\omega\Delta t})-F^{Hybrid}_{\beta-\frac{1}{2}}(\widehat{W}^{\omega\Delta t})\bigg) \\
&={W}^{0}_{\beta}+{\Delta t}\bigg( \mathcal{R}+\frac{\Delta t}{2} \mathcal{R}\frac{\partial \mathcal{R}}{\partial \mathcal{W}} \\
& \text{ }\text{ }\text{ }\text{ }+\mathcal{O}(\frac{\Delta t^2}{\Delta x},\frac{\Delta t^3}{\Delta x^2},\Delta t\Delta x^{p-2},\Delta t^2 \Delta x^{p-3},\Delta x^{p-1})\bigg).
\end{aligned}
\end{equation}
Thus the error $e(W^{\Delta t}_{\beta})$ may be formulated such as
\begin{equation}
\begin{aligned}
    e(W^{\Delta t}_{\beta})&=\mathcal{W}^{0}_{\beta}+\Delta t\frac{\partial \mathcal{W}}{\partial t}+\frac{\Delta t^2}{2}\frac{\partial^2 \mathcal{W}}{\partial t^2}+\mathcal{O}(\Delta t^3)-W^{\Delta t}_{\beta} \\
    &=\mathcal{O}(\Delta t^3,\frac{\Delta t^3}{\Delta x},\frac{\Delta t^4}{\Delta x^2},\Delta t\Delta x^{p-1},\Delta t^2\Delta x^{p-2},\Delta t^3 \Delta x^{p-3}).
\end{aligned}
\label{eq:error_beta_AION}
\end{equation}
Thanks to Eq.~\eqref{eq:error_beta_AION}),
and the stencil of the MUSCL reconstruction technique (see Eq.~\eqref{eq:error_parabolic_AION}),
the fluxes $F_{\beta-\frac{1}{2}}(W^{\Delta t})$ and $F_{\beta-\frac{1}{2}}(\widehat{W}^{2\omega\Delta t})$ may be formulated as
\begin{equation}
\begin{aligned}
    F^{Hybrid}_{\beta-\frac{1}{2}}(\widehat{W}^{2\omega\Delta t})&=\mathcal{F}_{\beta-\frac{1}{2}}+\Delta t \mathcal{R} \frac{\partial \mathcal{F}_{\beta-\frac{1}{2}}}{\partial \mathcal{W}}+ \mathcal{O}(\Delta t^2,\frac{\Delta t^3}{\Delta x},\frac{\Delta t^4}{\Delta x^2},\Delta t\Delta x^{p-1},\Delta t^2\Delta x^{p-2},\Delta t^3 \Delta x^{p-3},\Delta x^p)
%    F_{\beta-\frac{1}{2}}({W}^{\Delta t})&= \mathcal{F}_{\beta-\frac{1}{2}}+ a_{10}\Delta t^3+b_{10}\frac{\Delta t^3}{\Delta x}+c_{10}\frac{\Delta t^4}{\Delta x^2}+d_{10}\Delta t\Delta x^{p-1}\\
%    &\text{ }\text{ }\text{ }\text{ }+e_{10}\Delta t^2\Delta x^{p-2}+g_{10}\Delta t^3\Delta x^{p-3}+h_{10}\Delta x^p
\end{aligned}
\label{eq:error_flux_beta-1/2_2_AION}
\end{equation}
The state $W^{2\Delta t}_{\beta}$ may be formulated, thanks to Eqs.~\eqref{eq:error_flux_beta-1/2_2_AION}, \eqref{eq:error_flux_beta_2_AION}, \eqref{eq:error_flux_beta_AION}, and~\eqref{eq:error_beta_AION}, such as
\begin{equation}
\begin{aligned}
{W}^{2\Delta t}_{\beta}&={W}^{\Delta t}_{\beta}+\frac{\Delta t}{\Delta x} \bigg( \frac{3}{2}F^{Hybrid}_{\beta+\frac{1}{2}}(\widehat{W}^{2\omega\Delta t})-\frac{1}{2}F_{\beta+\frac{1}{2}}({W}^{0})-F^{Hybrid}_{\beta-\frac{1}{2}}(\widehat{W}^{2\omega\Delta t})\bigg). \\
&=\mathcal{W}^{\Delta t}_{\beta}+\mathcal{O}(\Delta t^3,\frac{\Delta t^3}{\Delta x},\frac{\Delta t^4}{\Delta x^2},\Delta t\Delta x^{p-1},\Delta t^2\Delta x^{p-2},\Delta t^3 \Delta x^{p-3}) \\
&\text{ }\text{ }\text{ }\text{ }+{\Delta t}\bigg( \mathcal{R}+\frac{3}{2}\Delta t \mathcal{R}\frac{\partial \mathcal{F}_{\beta+\frac{1}{2}}/\Delta x}{\partial \mathcal{W}}-\frac{1}{2}\Delta t \mathcal{R}\frac{\partial \mathcal{F}_{\beta-\frac{1}{2}}/\Delta x}{\partial \mathcal{W}} \\
&\text{ }\text{ }\text{ }\text{ }+\mathcal{O}(\frac{\Delta t^2}{\Delta x},\frac{\Delta t^3}{\Delta x^2},\frac{\Delta t^4}{\Delta x^3},\Delta t\Delta x^{p-2},\Delta t^2 \Delta x^{p-3},\Delta t^3 \Delta x^{p-4},\Delta x^{p-1})
\bigg).
\end{aligned}
\end{equation}
and the local error $e({W}^{2\Delta t}_{\beta})$ may be formulated such as
\begin{equation}
\begin{aligned}
    e(W^{2\Delta t}_{\beta})&=\mathcal{W}^{\Delta t}_{\beta}+\Delta t\frac{\partial \mathcal{W}}{\partial t}+\frac{\Delta t^2}{2}\frac{\partial^2 \mathcal{W}}{\partial t^2}+\mathcal{O}(\Delta t^3)-W^{2\Delta t}_{\beta} \\
    &=\bigg(\frac{1}{2}\frac{\partial^2 \mathcal{W}}{\partial t^2}-\frac{3}{2} \mathcal{R}\frac{\partial \mathcal{F}_{\beta+\frac{1}{2}}/\Delta x}{\partial \mathcal{W}}+\frac{1}{2} \mathcal{R}\frac{\partial \mathcal{F}_{\beta-\frac{1}{2}}/\Delta x}{\partial \mathcal{W}} \bigg)\Delta t^2 \\
    &\text{ }\text{ }\text{ }\text{ }+\mathcal{O}({\Delta t^3},\frac{\Delta t^3}{\Delta x},\frac{\Delta t^4}{\Delta x^2},\frac{\Delta t^5}{\Delta x^3},\Delta t\Delta x^{p-1},\Delta t^2\Delta x^{p-2},\Delta t^3 \Delta x^{p-3},\Delta t^4 \Delta x^{p-4})\\
    &=\mathcal{O}({\Delta t^2},\frac{\Delta t^3}{\Delta x},\frac{\Delta t^4}{\Delta x^2},\frac{\Delta t^5}{\Delta x^3},\Delta t\Delta x^{p-1},\Delta t^2\Delta x^{p-2},\Delta t^3 \Delta x^{p-3},\Delta t^4 \Delta x^{p-4}).
\end{aligned}
\label{eq:error_beta_2dt_AION}
\end{equation}
It appears that according to CFL condition is possible to link $\Delta t$ and $\Delta x$ in case of hyperbolic equation such as $\Delta x \simeq \Delta t$ and
then the local numerical error performed until $t=2\Delta t$ on cell $\beta$ of class rank $0$ is $O(\Delta t^2,\Delta x^p)$
whereas the local numerical error at cells of class rank $1$ is $O(\Delta t^2,\Delta x^p)$.
It appears that locally the temporal accuracy is conserve in hybrid part of AION scheme too.
In the following section, the influence of local numerical error due to time synchronisation in hybrid of AION scheme on global error will be tested.

==> Makefile <==
SRC 	 = TA
BIBLIO 	 = biblio.bib
LATEX 	 = pdflatex # -interaction=batchmode
BIBTEX 	 = bibtex -terse
CHAPTERS = 1_intro.tex \
		   2_TA_Heun.tex \
		   2_TA_Heun_b.tex \
		   3_TA_AION.tex \
		   4_validation.tex \
		   6_section.tex \
		   7_Conclusion.tex \
		   TA.tex

all: ${SRC}.pdf

${SRC}.pdf: ${SRC}.tex ${BIBLIO} ${CHAPTERS}
	@echo ' >>> Building paper'
	@${LATEX} ${SRC}.tex #> tex.log
	@${BIBTEX} ${SRC} #> bib.log
	@${BIBTEX} ${SRC} #> bib.log
	@${LATEX} ${SRC}.tex #> tex.log
	@${LATEX} ${SRC}.tex #> tex.log
	@make clean

clean:
	@rm -f ${SRC}.{dvi,ps,aux,log,bbl,blg,out,spl,toc,lot,lof} *.log

plot:
	@echo ' >>> Making all plots'
	@python makePlot.py

data:
	@echo ' >>> Making all data'
	@python makeData.py

